Read It, Don't Watch It: Captioning Bug Recordings Automatically

Screen recordings of mobile applications are easy to capture and include a wealth of information, making them a popular mechanism for users to inform developers of the problems encountered in the bug reports. However, watching the bug recordings and efficiently understanding the semantics of user actions can be time-consuming and tedious for developers. Inspired by the conception of the video subtitle in movie industry, we present a lightweight approach CAPdroid to caption bug recordings automatically. CAPdroid is a purely image-based and non-intrusive approach by using image processing and convolutional deep learning models to segment bug recordings, infer user action attributes, and generate subtitle descriptions. The automated experiments demonstrate the good performance of CAPdroid in inferring user actions from the recordings, and a user study confirms the usefulness of our generated step descriptions in assisting developers with bug replay.

==> tmp.tex <==
% video noise
% https://www.premiumbeat.com/blog/understanding-film-video-image-noise/

% Some good analyse of video segmentation methods
% Temporal video segmentation: A survey
% https://www.csie.ntu.edu.tw/~r96944046/paper/MMAI/Temporal%20video%20segmentation%20-%20a%20survey.pdf
% - The main disadvantage of this method is that it is not able to distinguish between a large change in a small area and a small change in a large area. For example, cuts are misdetected when a small part of the frame undergoes a large, rapid change. Therefore, methods based on simple pixel comparison are sensitive to object and camera movements.
% - For example, if camera pans, a large number of pixels can be judged as changed, even though there is actually a shift with a few pixels.




\begin{algorithm}[t]
    \linespread{1.2}
    \footnotesize
    % \setstretch{1.4}
	\SetAlgoLined
	\SetNoFillComment
	\SetKwInOut{Input}{Inputs}
	\SetKwInOut{Output}{Output}
	\SetKwProg{TAP}{TAP}{}{}
	\SetKwProg{SCROLL}{SCROLL}{}{}
	\SetKwProg{INPUT}{INPUT}{}{}
	\Input{$obj$: GUI element object; \\ 
		$nbr$: GUI element's neighbor; \\
		$\alpha, \beta$: high- and low-confidence thresholds \\ $\qquad$ for GUI element information;}
	\Output{natural language description}
	\tcc{Generate $TAP$ description}
	\TAP{$(obj, nbr, \alpha, \beta)$}{
	    \tcc{High-confidence GUI element with text or caption information}
	    \uIf{(\textit{obj\textsubscript{text/caption}} $\neq$ \textit{NULL} and \textit{obj\textsubscript{confid}} $> \alpha$)}{
	        \textbf{return} ``Tap [\textit{obj\textsubscript{text}}] [\textit{obj\textsubscript{class}}]''
	    }
	    \tcc{Medium-confidence GUI element with text or caption information}
	    \uElseIf{(\textit{obj\textsubscript{text/caption}} $\neq$ \textit{NULL} and $\beta <$ \textit{obj\textsubscript{confid}} $< \alpha$)}{
	        \textbf{return} ``Tap [\textit{obj\textsubscript{text}}] [\textit{obj\textsubscript{class}}] at [\textit{obj\textsubscript{position}}]''
	    }
	    \tcc{Low-confidence GUI element, or no text or caption recognized}
	    \Else{
	        \textbf{return} ``Tap [\textit{obj\textsubscript{class}}] [\textit{nbr\textsubscript{relation}}] [\textit{nbr\textsubscript{text}}]''
	    }
	}
	
	\tcc{Generate $SCROLL$ description}
	\SCROLL{$(obj)$}{
	    \uIf{(\textit{obj\textsubscript{text}} == \textit{NULL})}{
	        \textbf{return} ``Scroll [\textit{direction}] [\textit{offset}] of the screen''
	    }
	    \Else{
	        \textbf{return} ``Scroll [\textit{direction}] [\textit{offset}] of the screen to  [\textit{obj\textsubscript{text}}]''
	    }
	}
	
	\tcc{Generate $INPUT$ description}
	\INPUT{$(obj, nbr, \alpha)$}{
	    \uIf{(\textit{obj\textsubscript{text/caption}} $\neq$ \textit{NULL} and \textit{obj\textsubscript{confid}} $> \alpha$)}{
	        \textbf{return} ``Input [\textit{text}] in the [\textit{obj\textsubscript{text}}] edittext''
	    }
	    \Else{
	        \textbf{return} ``Input [\textit{text}] in the edittext [\textit{nbr\textsubscript{relation}}] [\textit{nbr\textsubscript{text}}]''
	    }
	}
	\caption{Natural Language Generation \chen{This algorithm is not very useful, why not get a table to summarizing different patterns for each action with a given example? Can show you one example of my another paper QTypist.}}
	\label{algorithm:nlg}
\end{algorithm}
